Confidence Interval Estimators for MOS Values

For the quantification of QoE, subjects often provide individual rating scores on certain rating scales which are then aggregated into Mean Opinion Scores (MOS). From the observed sample data, the expected value is to be estimated. While the sample average only provides a point estimator, confidence intervals (CI) are an interval estimate which contains the desired expected value with a given confidence level. In subjective studies, the number of subjects performing the test is typically small, especially in lab environments. The used rating scales are bounded and often discrete like the 5-point ACR rating scale. Therefore, we review statistical approaches in the literature for their applicability in the QoE domain for MOS interval estimation (instead of having only a point estimator, which is the MOS). We provide a conservative estimator based on the SOS hypothesis and binomial distributions and compare its performance (CI width, outlier ratio of CI violating the rating scale bounds) and coverage probability with well known CI estimators. We show that the provided CI estimator works very well in practice for MOS interval estimators, while the commonly used studentized CIs suffer from a positive outlier ratio, i.e., CIs beyond the bounds of the rating scale. As an alternative, bootstrapping, i.e., random sampling of the subjective ratings with replacement, is an efficient CI estimator leading to typically smaller CIs, but lower coverage than the proposed estimator.

==> _region_.tex <==
\message{ !name(estimators.tex)}
\message{ !name(estimators.tex) !offset(-2) }
\section{Confidence Interval Estimators for MOS}\label{sec:estimators}

\subsection{Problem Formulation}
Discrete rating scale with $k$ rating items leading to a multinominal
distribution which is the generalization of the binomial distribution. For a
certain test condition, $n$ users are rating the QoE on a discrete $k$-point
rating scale, e.g. $k=5$ for the commonly used 5-point Absolute Category Rating
(ACR) scale. Each scale item is selected with probability $p_i$ for
$i=1,\dots,k$. It is $\sum_{i=1}^k p_i = 1$.

The $n$ users rate the QoE as one of the $k$ categories, with each category
having a fixed probability $p_i$, the multinomial distribution gives the
probability of any particular combination of numbers $n_i$ of successes for the
various categories. It is $\sum_{i=1}^k n_i = n$.

\begin{equation}
P(N_1=n_1,\dots,N_k=n_k) = \frac{n!}{n_1! \cdots n_k!} p_1^{n_1}\cdots p_k^{n_k}
\label{eq:multinominal}
\end{equation}

In the QoE tests, we are interested in the rating of an arbitrary user. When $n=1$, it is the categorical distribution with $p_i$.

The true, but unknown mean value, i.e. the MOS, is then 
\begin{equation}
	\E[Y] = \frac{1}{k} \sum_{i=1}^k i p_i
\label{eq:unknownMOS}
\end{equation}
by interpreting the category rating scale as a linear scale. 

$Y$ is a random variable of the rating of the users. We observe a sample $y_1, \dots, y_n$ with $y_i \in \{1,\dots,k\}$.

In QoE tests, the number $n$ of users is typically not very high ($n=20$ or $n=30$, as recommended in some ITU-T standards), since a lot of test conditions are evaluated. 

From the samples $(n_1,\dots,n_k)$, i.e. the number of ratings per category, the MOS is estimated. Confidence intervals are the corresponding interval estimators for the mean value.

The problem is that exiting estimators do not work properly for small sample sizes (e.g. normal distribution assumption not valid) and that they violate the bounds of the confidence interval.

Bounded confidence interval, small sample size 



\subsection{Regular Normal and Student-T Approximation}
\hoss{Description of the computation of the confidence intervals can be a mix of programming code and proper formulas. }

standard formula

$y_i$ is the rating of user $i$

\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
ci.norm = mean(yi)+norminv([ci.alpha/2, 1-ci.alpha/2],0,1).*std(yi)/sqrt(n);
ci.studentT = mean(yi)+tinv([ci.alpha/2  1-ci.alpha/2],n-1).*std(yi)/sqrt(n);
\end{lstlisting}

\hoss{Can you simply limit the confidence interval to not violate the bounds? No, this would not be correct!}


\subsection{Using Binomial Proportions for Discrete Rating Scales}

\begin{itemize}
	\item The binomial distribution can be used as an upper bound distribution for user rating distributions. The binomial distribution leads to high standard deviations in QoE tests \cite{hossfeld2011sos}. The binomial distribution follows exactly the SOS hypothesis with parameter $a=1/m$ and $m+1$ rating scale items, for example $m=u-l=4$ in case of a 5-point ACR scale with bounds $l=1$ and $u=5$.
\item Let us consider $n$ users. Assume the user ratings follow a binomial distribution, $Y_i \sim \bino{m,p}$ with $l=0$ and $u=m$. Then, the sum of the user ratings follows also a binomial distribution. 
	\begin{equation}
	Y=\sum_{i=1}^n Y_i \sim \bino{\sum_{i=1}^n m,p}=\bino{n\cdot m,p}
	\end{equation}
	\item Due to differences among users, it may be $p_i \neq p_j$ for user $i$ and $j$. Due to the binomial sum variance inequality, we know the following. Thus, let us consider $Y=\sum_{i=1}^n Y_i$ which is not following a binomial distribution. Let us define $Z\sim \bino{n\cdot m,\bar{p}}$ with $\bar{p}=\frac{1}{n} \sum_{i=1}^n p_i$.
	\begin{equation}
	\Var[Y] < \Var[Z]
	\end{equation}
		\item Hence, the variance of $Z$ is an upper bound for QoE tests. Accordingly, we may use $Z$ to derive conservative confidence intervals.
\end{itemize}


Some approaches for binomial distributions

\verb|res(i,j)| indicates the confidence interval width of test condition $i$ and confidence estimator $j$

\verb|low(i,j)| is the lower confidence interval end; \verb|up(i,j)| is the upper bound

\begin{itemize}
	\item  Wald interval employing normal approximation 
	\hoss{Needs to be checked; performance is too bad for binomial case}
	\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% binomial proportion: Wald
z=norminv(1-ci.alpha/2,0,1);
mu=mean(yi)-1; m=4;
p=mu/m;
s = sqrt(p*(1-p)/n);
p1 = p-z*s;p2=p+z*s;
low(i,4)=p1*m+1; up(i,4)=p2*m+1;
res(i,4)=(up(i,4)-low(i,4))/2;


  \end{lstlisting}	
	\item  Wilson score interval with continuity correction
	
	\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]	
% binomial proportion: Wilson     
low(i,5)=max(1, (2*p*n*m + z2 - (1+z*sqrt(z2-1./(n*m) + 4*n*m*p*(1-p)+(4*p-2)) )  )/(2*(n*m+z2)) *m+1 );
up(i,5)=min(m+1, (2*p*n*m + z2 + (1+z*sqrt(z2-1./(n*m) + 4*n*m*p*(1-p)+(4*p-2)) )  )/(2*(n*m+z2)) *m+1 );
res(i,5)=(up(i,5)-low(i,5))/2;
    \end{lstlisting}	
   
	
	\item  Clopper-Pearson (using beta distribution)
\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% binomial proportion: clopper-pearson using beta
numSuc=sum(yi-1);trials=n*m;
low(i,6) = max(1, betainv(ci.alpha/2,numSuc, trials-numSuc+1) *m + 1);
up(i,6) = min(m+1, betainv(1-ci.alpha/2,numSuc+1, trials-numSuc) *m + 1);
res(i,6)=(up(i,6)-low(i,6))/2;    
   \end{lstlisting}	
\end{itemize}

Approximate results for binomial proportions are sometimes more useful than exact results because of the inherent conservative calculation of exact methods \cite{agresti1998approximate}.

\subsection{Simultaneous Confidence Intervals for Multinomial Distribution}
Computing Exact Confidence Coefficients of Simultaneous Confidence Intervals for Multinomial Proportions and their Functions \cite{jin2013computing}
\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% simultaneous confidence intervalls
di=1:5;
xi = hist(yi,di);
a = chi2inv(1-ci.alpha,length(di)-1);  % a = chi^2(1-alpha,d-1)
a = chi2inv(1-ci.alpha/length(di),1); % bonferroni
scim = sum((1:5).*xi/n);
low(i,7)=scim-sqrt(a/n.*(sum((1:5).^2.*xi/n)- (sum((1:5).*xi/n)).^2 ));
up(i,7)=scim+sqrt(a/n.*(sum((1:5).^2.*xi/n)- (sum((1:5).*xi/n)).^2 ));
res(i,7)=(up(i,7)-low(i,7))/2;    
\end{lstlisting}


%\subsection{Confidence Intervals using Truncated Normal Distributions}
%An own idea

\subsection{Bayesian Approach for Multinomial Distributions}
\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% Jeffreys interval
if numSuc==0, low(i,8)=1;
else
    low(i,8)=betainv(ci.alpha/2,numSuc+1/2, trials-numSuc+1/2)*m+1;
end
if numSuc==trials, up(i,8)=5;
else
    up(i,8)=betainv(1-ci.alpha/2,numSuc+1/2, trials-numSuc+1/2)*m+1;
end
res(i,8)=(up(i,8)-low(i,8))/2;
\end{lstlisting}


\subsection{Bootstrap Confidence Intervals}
\message{ !name(estimators.tex) !offset(-152) }


==> background.tex <==
\section{Background}\label{sec:background}
\hoss{The notation is not consistent so far, we should introduce a table with the notation and variables used.}

For the sake of readability, we briefly state the definitions and theorems used to derive CI estimators. Table \ref{tab:notion} provides a summary of the notation and variables used throughout the paper. 

\subsection{Definition and Theorems}
\martin{Since we're not proving any theorem here, maybe we should rename all
  this to ``Definitions and assumptions''?}
  
\lea{Is this ``theorem'' regarding CIs actually a definition? Another question: do we really need subsection B here on desirable properties? Given the space limitations, I think we should cut back on textbook stuff to free up room needed to fit to 6 pgs. I would keep just this subsection, but it then doesn't need to be a subsection...}
  
\martin{I agree on the ``Desirable properties'' section. I'd drop it. We can see
about the textbook stuff if we need to further cut; we could keep it very
succint, if need be.}
\begin{theorem}[Confidence interval]
Let $X$ be a random sample from a probability distribution with statistical parameter $\theta$, which is a quantity to be estimated. A confidence interval for the parameter $\theta$, with confidence level $\gamma$ is the interval $[u(X), v(X)]$ which satisfies 
\begin{equation}
\forall \theta: P(u(X)<\theta<u(X))\geq \gamma \, .
\label{eq:ci}
\end{equation}
\end{theorem}

\begin{theorem}[Central limit theorem] Let $\{X_1, \dots, X_n\}$ be a random sample of size $n$ with independent, identically distributed random variables $X_i$. 

  For large samples, the sample mean has a normal distribution with mean equal
  to $\E[X]$ and variance equal to $\Var[X]/n$.

\begin{equation}
\xbar \sim N(\E[X],\Var[X]/n)
\label{eq:clt}
\end{equation}
\end{theorem}

The CLT implies that the sample mean can be rescaled to a standard normal
distribution with expected value 0 and variance equal to 1.
\begin{equation}
\frac{\xbar-\mu}{\sigma/\sqrt{n}} \sim N(0,1)
\label{eq:}
\end{equation}

This allows to derive CIs for mean values with $P(Z \leq -z) =
P(Z \geq z) = \gamma/2$ and $Z \sim N(0,1)$. For $\gamma=1-\alpha=0.95$, it is
$z \approx 1.96$.
\begin{align}
& P(-z \leq \frac{\xbar-\mu}{\sigma/\sqrt{n}} \leq z) = \\ 
& P(\xbar -z \sigma/\sqrt{n} \leq \mu \leq \xbar + z \sigma/\sqrt{n} ) \quad \geq \gamma 
\end{align}

\begin{theorem}[Confidence intervals for mean values] 
The confidence interval for the unknown mean value $\mu$ can be derived using the sample mean $\xbar$ and the 
standard error of sample mean, $S/\sqrt{n}$
%sample variance $S^2$ 
for a sample of size $n$. Thereby $z$ is the $\gamma/2$-quantile of the standard normal distribution $N(0,1)$.
\begin{equation}
\xbar \pm z \cdot \frac{S}{\sqrt{n}}
\label{eq:ciMean}
\end{equation}
\end{theorem}

The size of the confidence interval depends on the sample size and the standard
deviation of the study groups. If the sample size is large, this leads to "more
confidence" and a narrower confidence interval. If the confidence interval is
wide, this may mean that the sample is small. If the dispersion is high, the
conclusion is less certain and the confidence interval becomes wider.

\subsection{Desirable Properties of Confidence Intervals}

Confidence level: how reliable is the interval

Confidence interval width: how meaningful is this CI

Exact confidence intervals vs. approximate confidence intervals

Computational effort

\input{notion}

==> estimators.tex <==
\section{Confidence Interval Estimators for MOS}\label{sec:estimators}

\subsection{Problem Formulation}
\martin{A ``feeling'' note: I'd tend to speak of ``quality'' rather than ``QoE''
  throughout here} \lea{OK, I changed it to quality.} We assume we have a
discrete rating scale with $k$ rating items, leading to a multinominal
distribution, which is a generalization of the binomial distribution. For a
certain test condition, $n$ users rate the quality on a discrete $k$-point
rating scale, e.g., $k=5$ for the commonly used 5-point ACR scale. Each scale
item is selected with probability $p_i$ for $i=1,\dots,k$; $\sum_{i=1}^k p_i =
1$.

The $n$ users rate quality as one of the $k$ categories. Samples
$(n_1,\dots,n_k)$ indicate the number of ratings obtained per category, with
$\sum_{i=1}^k n_i = n$ (i.e., each user has provided one rating). With each
category having a fixed probability $p_i$, the multinomial distribution gives
the probability of any particular combination of numbers $n_i$ of successes for
the various categories.

\begin{equation}
P(N_1=n_1,\dots,N_k=n_k) = \frac{n!}{n_1! \cdots n_k!} p_1^{n_1}\cdots p_k^{n_k}
\label{eq:multinominal}
\end{equation}

In the QoE tests, we are interested in the rating of an arbitrary user. When
$n=1$, it is the categorical distribution with $p_i$. The true, but unknown mean
value, i.e. the MOS, is then
\begin{equation}
	\E[Y] = \frac{1}{k} \sum_{i=1}^k i p_i
\label{eq:unknownMOS}
\end{equation}

by interpreting the category rating scale as a linear scale. 

We denote $Y$ as a random variable of the rating of the users. We observe a
sample $y_1, \dots, y_n$ with $y_i \in \{1,\dots,k\}$. As previously stated, in
subjective QoE tests, the number $n$ of users is typically not very high. From
the samples $(n_1,\dots,n_k)$, the MOS is estimated, with CIs being the
corresponding interval estimators for the mean value. However, given the use of
a bounded rating scale and small sample size, existing estimators do not work
properly (e.g., normality assumptions no longer hold), and they violate the
bounds of the confidence interval.\martin{Shouldn't this read ``violate the
  bounds of the rating scale''?}


\subsection{Regular Normal and Student-T Approximation}
\hoss{Description of the computation of the confidence intervals can be a mix of programming code and proper formulas. }
\martin{I think just having the math would be more readable and succint. We
  could put the matlab code in pastebin (anonymized) and link to it. We can
  later move it to a github gist when we do the camera ready}
standard formula

$y_i$ is the rating of user $i$

\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
ci.norm = mean(yi)+norminv([ci.alpha/2, 1-ci.alpha/2],0,1).*std(yi)/sqrt(n);
ci.studentT = mean(yi)+tinv([ci.alpha/2  1-ci.alpha/2],n-1).*std(yi)/sqrt(n);
\end{lstlisting}

\hoss{Can you simply limit the confidence interval to not violate the bounds? No, this would not be correct!}


\subsection{Using Binomial Proportions for Discrete Rating Scales}

\begin{itemize}
\item The binomial distribution can be used as an upper bound distribution for
  user rating distributions. The binomial distribution leads to high standard
  deviations in QoE tests \cite{hossfeld2011sos}. The binomial distribution
  follows exactly the SOS hypothesis with parameter $a=1/m$ and $m+1$ rating
  scale items, for example $m=u-l=4$ in case of a 5-point ACR scale with bounds
  $l=1$ and $u=5$.
\item Let us consider $n$ users. Assume the user ratings follow a binomial distribution, $Y_i \sim \bino{m,p}$ with $l=0$ and $u=m$. Then, the sum of the user ratings follows also a binomial distribution. 
	\begin{equation}
	Y=\sum_{i=1}^n Y_i \sim \bino{\sum_{i=1}^n m,p}=\bino{n\cdot m,p}
	\end{equation}
	\item Due to differences among users, it may be $p_i \neq p_j$ for user $i$ and $j$. Due to the binomial sum variance inequality, we know the following. Thus, let us consider $Y=\sum_{i=1}^n Y_i$ which is not following a binomial distribution. Let us define $Z\sim \bino{n\cdot m,\bar{p}}$ with $\bar{p}=\frac{1}{n} \sum_{i=1}^n p_i$.
	\begin{equation}
	\Var[Y] < \Var[Z]
	\end{equation}
		\item Hence, the variance of $Z$ is an upper bound for QoE tests. Accordingly, we may use $Z$ to derive conservative confidence intervals.
\end{itemize}


Some approaches for binomial distributions

CI estimation for binomial distributions has drawn attention in literature and several suggestions have been provided. There are a couple of works which compare the CI estimators for binomial proportions \cite{pires2008interval,vollset1993confidence,brown2001interval,newcombe2012confidence}. For example, \cite{brown2001interval} suggest Wilson interval and Jeffreys prior interval for small $n$. The standard Wald confidence interval howvers is not recommended \cite{agresti1998approximate}.

\verb|res(i,j)| indicates the confidence interval width of test condition $i$ and confidence estimator $j$

\verb|low(i,j)| is the lower confidence interval end; \verb|up(i,j)| is the upper bound

\begin{itemize}
	\item  Wald interval employing normal approximation 
	
	The normal theory approximation of a confidence interval for a proportion is
known as the Wald interval
	
	\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% binomial proportion: Wald
z=norminv(1-ci.alpha/2,0,1);
mu=mean(yi)-1; m=4;
p=mu/m;
s = sqrt(p*(1-p)/n);
p1 = p-z*s;p2=p+z*s;
low(i,4)=p1*m+1; up(i,4)=p2*m+1;
res(i,4)=(up(i,4)-low(i,4))/2;


  \end{lstlisting}	
	\item  Wilson score interval with continuity correction
	
	\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]	
% binomial proportion: Wilson     
low(i,5)=max(1, (2*p*n*m + z2 - (1+z*sqrt(z2-1./(n*m) + 4*n*m*p*(1-p)+(4*p-2)) )  )/(2*(n*m+z2)) *m+1 );
up(i,5)=min(m+1, (2*p*n*m + z2 + (1+z*sqrt(z2-1./(n*m) + 4*n*m*p*(1-p)+(4*p-2)) )  )/(2*(n*m+z2)) *m+1 );
res(i,5)=(up(i,5)-low(i,5))/2;
    \end{lstlisting}	
   
	
	\item  Clopper-Pearson (using beta distribution)
	\cite{clopper1934use}  is the central exact interval 
	
\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% binomial proportion: clopper-pearson using beta
numSuc=sum(yi-1);trials=n*m;
low(i,6) = max(1, betainv(ci.alpha/2,numSuc, trials-numSuc+1) *m + 1);
up(i,6) = min(m+1, betainv(1-ci.alpha/2,numSuc+1, trials-numSuc) *m + 1);
res(i,6)=(up(i,6)-low(i,6))/2;    
   \end{lstlisting}	
\end{itemize}

Approximate results for binomial proportions are sometimes more useful than exact results because of the inherent conservative calculation of exact methods \cite{agresti1998approximate}.

\subsection{Simultaneous Confidence Intervals for Multinomial Distribution}
Computing Exact Confidence Coefficients of Simultaneous Confidence Intervals for Multinomial Proportions and their Functions \cite{jin2013computing}
\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% simultaneous confidence intervalls
di=1:5;
xi = hist(yi,di);
a = chi2inv(1-ci.alpha/length(di),1); % bonferroni
scim = sum((1:5).*xi/n);
low(i,7)=scim-sqrt(a/n.*(sum((1:5).^2.*xi/n)- (sum((1:5).*xi/n)).^2 ));
up(i,7)=scim+sqrt(a/n.*(sum((1:5).^2.*xi/n)- (sum((1:5).*xi/n)).^2 ));
res(i,7)=(up(i,7)-low(i,7))/2;    
\end{lstlisting}


%\subsection{Confidence Intervals using Truncated Normal Distributions}
%An own idea

\subsection{Jeffreys Interval: Bayesian Approach for Binomial Proportions}
Another exact method is a Bayesian credibility interval which guarantees a mean coverage probability of $\gamma$ under the specified prior distribution. \cite{brown2001interval} have chosen the Jeffreys prior \cite{jeffreys1998theory}. 



\begin{lstlisting}[backgroundcolor=\color{MatlabCellColour}]
% Jeffreys interval
if numSuc==0, low(i,8)=1;
else
    low(i,8)=betainv(ci.alpha/2,numSuc+1/2, trials-numSuc+1/2)*m+1;
end
if numSuc==trials, up(i,8)=5;
else
    up(i,8)=betainv(1-ci.alpha/2,numSuc+1/2, trials-numSuc+1/2)*m+1;
end
res(i,8)=(up(i,8)-low(i,8))/2;
\end{lstlisting}


\subsection{Bootstrap Confidence Intervals}
The non-parametric bootstrap method was introduced by Efron introduced by \cite{efron1992bootstrap} uses solely the empirical distribution of the observed sample. 

We use the Matlab implementation with the `Bias corrected and accelerated percentile' method. 



==> garbage.tex <==
\clearpage 
\clearpage 

\section*{\textcolor{orange}{\huge{Collection of Stuff}}}

%\begin{tikzpicture}
%\tikzset{level distance=60pt}
% \Tree 	[.MOS~CIs [.approximation normal student-t bootstrap ] [.binomial Wald Wilson Clopper-Pearson  ]
% ]

%\end{tikzpicture}	

%\begin{table}%
%\caption{Notion of variables frequently used in this paper.}\label{tab:notion}
%\begin{tabularx}{\columnwidth}{lX}
%\toprule
%Notion & Description \\
%\midrule
%$l$ & lower bound of rating scale\\
%$u$ & upper bound of rating scale \\
%$m$ & width of discrete rating scales, i.e. $m=u-l$\\
%$n$ & number of subjects conducting the QoE study\\
%$k$ & number of test conditions evaluated per user\\
%$Y$ & user rating distribution (RV) for a certain test condition\\
%\bottomrule
%\end{tabularx}
%
%\end{table}
%
%\begin{table}%
%\caption{Summary of confidence interval approaches for discrete rating scales.}\label{tab:summaryDiscrete}
%\begin{tabular}{llll}
%\toprule
%Approach & formulae & efficiency & coverage \\
%\midrule
%Wald & & & \\
%Clopper-Pearson & & & \\
%\bottomrule
%\end{tabular}
%
%\end{table}






\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/extremeperformanceCDF}%
\caption{\extremecase Single run. \emph{extremeperformanceCDF.pdf from 15-Jan-2018 00:02:55}}%
\label{fig:extremeperformanceCDF}%
%\end{figure}
%
%\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/extremeperformanceBars}%
\caption{\extremecase Single run. \emph{extremeperformanceBars.pdf from 15-Jan-2018 00:02:26}}%
\label{fig:extremeperformanceBars}%
\end{figure}

\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/discreteperformanceBars}%
\caption{Results for a real use case: image QoE. Variance is lower than for the binomial case (can be checked with SOS parameter $a=0.16 < 0.25$. \newline \emph{discreteperformanceBars.pdf from 15-Jan-2018 00:07:53}}%
\label{fig:discreteperformanceBars}%
\end{figure}


\begin{figure}%
\centering%
\includegraphics[width=\figwidth]{figs/randComputation}%
\caption{The drawback of bootstrapping is the increased computation time. But this is not relevant in practice for QoE tests! \newline \emph{randComputation.pdf from 22-Jan-2018 00:45:55}}%
\label{fig:randComputation}%
\end{figure}

											


\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/randefficiency}%
\caption{\randcase Instead of the extreme case, we can also investigate the random case, i.e. users are rating randomly. This is already quite extreme for QoE tests and an indicator that the test is not working in practice. \newline \emph{randefficiency.pdf from 22-Jan-2018 00:16:38}}%
\label{fig:randefficiency}%
\centering%
\includegraphics[width=\figwidth]{figs/randoutlierRatio}%
\caption{\randcase \newline \emph{randoutlierRatio.pdf from 22-Jan-2018 00:16:40}}%
\label{fig:randoutlierRatio}%
\centering%
\includegraphics[width=\figwidth]{figs/randciWidthComp}%
\caption{\randcase \newline \emph{randciWidthComp.pdf from 22-Jan-2018 00:16:42}}%
\label{fig:randciWidthComp}%
\end{figure}



\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/test}%
\caption{\newline \emph{test.pdf from 22-Jan-2018 19:07:56}}%
\label{fig:test}%
\end{figure}


%%%%%%%%%%%%%%% Coverage %%%%%%%%%%%%%%% 
\subsubsection{Coverage of Estimators}
\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialefficiency}%
\caption{\binocase This indicates the coverage probability of the confidence interval (for the known real binomial values).\newline \emph{binomialefficiency.pdf from 15-Jan-2018 00:44:45}}%
\label{fig:binomialefficiency}%
%\end{figure}
%\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialLowVarianceefficiency}%
\caption{\lowvarcase Outlier ratio is zero for all CI estimators. \newline \emph{binomialLowVarianceefficiency.pdf from 15-Jan-2018 01:47:23}}%
\label{fig:binomialLowVarianceefficiency}%
\centering%
\includegraphics[width=\figwidth]{figs/extremeefficiency}%
\caption{\extremecase \newline \emph{extremeefficiency.pdf from 21-Jan-2018 23:55:31}}%
\label{fig:extremeefficiency}%
%%
\end{figure}


%%%%%%%%%%%%%%% Outlier Ratio %%%%%%%%%%%%%%% 
\subsubsection{Outlier Ratio}
There are $n=20$ subjects who rate $m=100$ test conditions on a $k=5$-point rating scale.

The simulations are repeated $r=200$ times.

\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialoutlierRatio}%
\caption{\binocase \newline \emph{binomialoutlierRatio.pdf from 15-Jan-2018 01:15:56}}%
\label{fig:binomialoutlierRatio}%
%%%
\centering%
\includegraphics[width=\figwidth]{figs/binomialLowVarianceoutlierRatio}%
\caption{\lowvarcase Outlier ratio is zero for all CI estimators. \newline \emph{binomialLowVarianceefficiency.pdf from 15-Jan-2018 01:47:23}}%
\label{fig:binomialLowVarianceefficiency}%
\centering%
\includegraphics[width=\figwidth]{figs/extremeoutlierRatio}%
\caption{\extremecase \newline \emph{extremeoutlierRatio.pdf from 21-Jan-2018 23:55:34}}%
\label{fig:extremeoutlierRatio}%
\end{figure}


%%%%%%%%%%%%%%% CI Width %%%%%%%%%%%%%%% 
\subsubsection{CI Width}
\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialciWidthComp}%
\caption{\binocase \newline \emph{binomialciWidthComp.pdf from 15-Jan-2018 01:49:01}}%
\label{fig:binomialciWidthComp}%
\centering%
\includegraphics[width=\figwidth]{figs/binomialLowVarianceciWidthComp}%
\caption{\lowvarcase \newline \emph{binomialLowVarianceciWidthComp.pdf from 15-Jan-2018 01:49:01}}%
\label{fig:binomialLowVarianceciWidthComp}%
\centering%
\includegraphics[width=\figwidth]{figs/extremeciWidthComp}%
\caption{\extremecase \newline \emph{extremeciWidthComp.pdf from 21-Jan-2018 23:55:35}}%
\label{fig:extremeciWidthComp}%
\end{figure}




\subsubsection{Single Example Run for Binomial Distributions}
%%%%%%%%%%%%%% Single Run %%%%%%%%%%%%%%%%
\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialperformanceCDF}%
\caption{Binomial case.  We generate $m=100$ test conditions which cover mean values from 1 to 5. There are $n=20$ subjects rating the TCs. Two CDFs lead to much higher CI widths, Wald and simultaneous CIs. The other estimators show similar behavior. A close look reveals that bootstrap, Clopper-Pearson, Wilson have the same shape, while student-t, normal, Jeffrey reach higher maximum CI widths. Please note that this is a single run only. We need to repeat the simulation run. \newline \emph{binomialperformanceCDF.pdf from 14-Jan-2018 23:44:11}}%
\label{fig:binomialperformanceCDF}%
%\end{figure}
%
%\begin{figure}[h]%
\centering%
\includegraphics[width=\figwidth]{figs/binomialperformanceBars}%
\caption{Binomial case. Results are summarized in this plot. Please note that this is a single run only. We need to repeat the simulation for many runs. \newline \emph{binomialperformanceBars.pdf from 14-Jan-2018 23:43:21}}%
\label{fig:binomialperformanceBars}%
\end{figure}

